Transfer of Reinforcement Learning-Based Controllers from Model- to Hardware-in-the-Loop

The process of developing control functions for embedded systems is resource-, time-, and data-intensive, often resulting in sub-optimal cost and solutions approaches. Reinforcement Learning (RL) has great potential for autonomously training agents to perform complex control tasks with minimal human intervention. Due to costly data generation and safety constraints, however, its application is mostly limited to purely simulated domains. To use RL effectively in embedded system function development, the generated agents must be able to handle real-world applications. In this context, this work focuses on accelerating the training process of RL agents by combining Transfer Learning (TL) and X-in-the-Loop (XiL) simulation. For the use case of transient exhaust gas re-circulation control for an internal combustion engine, use of a computationally cheap Model-in-the-Loop (MiL) simulation is made to select a suitable algorithm, fine-tune hyperparameters, and finally train candidate agents for the transfer. These pre-trained RL agents are then fine-tuned in a Hardware-in-the-Loop (HiL) system via TL. The transfer revealed the need for adjusting the reward parameters when advancing to real hardware. Further, the comparison between a purely HiL-trained and a transferred agent showed a reduction of training time by a factor of 5.9. The results emphasize the necessity to train RL agents with real hardware, and demonstrate that the maturity of the transferred policies affects both training time and performance, highlighting the strong synergies between TL and XiL simulation.

==> acronyms.tex <==
% Acronyms
\RequirePackage{xstring}
\RequirePackage{xparse}
\RequirePackage{acro}
\makeatletter
\@ifpackagelater{acro}{2019/02/17}{
	% work around bug in 2019/02/17
	\NewDocumentCommand\acrodef{mO{#1}mG{}}{\DeclareAcronym{#1}{short={#2}, long={#3}, foreign-plural={}, #4}}
}{
	\NewDocumentCommand\acrodef{mO{#1}mG{}}{\DeclareAcronym{#1}{short={#2}, long={#3}, #4}}
}
\makeatother
\acrodef{AI}{Artificial Intelligence}
\acrodef{API}{Application Programming Interface}
\acrodef{CAN}{Controller Area Network}
\acrodef{DDPG}{Deep Deterministic Policy Gradients}
\acrodef{DI}{Direct Injection}
\acrodef{DQN}{Deep Q-Network}
\acrodef{ECU}{Engine Control Unit}
\acrodef{EGR}{Exhaust Gas Recirculation}
\acrodef{GAE}{Generalized Advantage Estimation}
\acrodef{HiL}{Hardware-in-the-Loop}
\acrodef{HP}{High-Pressure}
\acrodef{IO}{Input/Output}
\acrodef{KL}{Kullback-Leibler}
\acrodef{LP}{Low-Pressure}
\acrodef{LSU}{Lambda-Sensor-Unit}
\acrodef{MDP}{Markov Decision Process}
\acrodef{MiL}{Model-in-the-Loop}
\acrodef{ML}{Machine Learning}
\acrodef{MPC}{Model-Predictive Control}
\acrodef{MVEM}{Mean Value Engine Model}
\acrodef{NN}{Neural Network}
\acrodef{OEM}{Original Equipment Manufacturer}
\acrodef{PG}{Policy Gradient}
\acrodef{PID}{proportional-integral-derivative}
\acrodef{PPO}{Proximal Policy Optimization}
\acrodef{PWM}{Pulse Width Modulation}
\acrodef{RDE}{Real Driving Emissions}
\acrodef{RL}{Reinforcement Learning}
\acrodef{RWD}{Rear Wheel Drive}
\acrodef{SCR}{Selective Catalytic Reduction}
\acrodef{SiL}{Software-in-the-Loop}
\acrodef{SGD}{Stochastic Gradient Descent}
\acrodef{TL}{Transfer Learning}
\acrodef{VCU}{Virtual Control Unit}
\acrodef{VGT}{Variable Geometry Turbocharger}
\acrodef{VM}{Virtual Machine}
\acrodef{WLTC}{Worldwide harmonized Light vehicles Test Cycle}
\acrodef{XiL}{X-in-the-Loop}
%\acrodef{API}{Application Programming Interface}
